Advanced Capsule Networks via Context Awareness

Capsule Networks (CN) offer new architectures for Deep Learning (DL) community. Though its effectiveness has been demonstrated in MNIST and smallNORB datasets, the networks still face challenges in other datasets for images with distinct contexts. In this research, we improve the design of CN (Vector version) namely we expand more Pooling layers to filter image backgrounds and increase Reconstruction layers to make better image restoration. Additionally, we perform experiments to compare accuracy and speed of CN versus DL models. In DL models, we utilize Inception V3 and DenseNet V201 for powerful computers besides NASNet, MobileNet V1 and MobileNet V2 for small and embedded devices. We evaluate our models on a fingerspelling alphabet dataset from American Sign Language (ASL). The results show that CNs perform comparably to DL models while dramatically reducing training time. We also make a demonstration and give a link for the purpose of illustration.

==> demonstration.tex <==
\subsection{Demonstration}
For the purpose of demonstration, we transfer trained weights of MobileNet V1, Capsule 32 V1 and Capsule 32 V2 from a GPU server to another computer (CPU 2.7GHz). 

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.95\textwidth]{img/7_1}
%   \caption{Demo of Capsule Networks vs Transfer Learning Models}
%   \label{fig:demo}
% \end{figure}

We developed an application that loads all of these weights at the runtime. We test these networks on ASL fingerspelling videos made by professional signers. 
Figure \ref{fig:demo} shows a screenshot of this application when the ASL sign is A. The red box indicates the area where the hand is detected. The box is plotted a little bigger so that the lines does not touch the hand for convenience of observing. The upper text shows a prediction from Capsule Networks and the lower text show another prediction from DeepNet (MobileNet V1). Recorded videos can be obtained via this link.

Since hands in these videos are moved around, we also built a detection technique to crop only the area surrounding the hand. Description of the technique is not included within this article to better focus on the main techniques.

==> figure1.tex <==
% \begin{figure}[p]
% \begin{subfigure}{\linewidth}
% \includegraphics[width=0.9\textwidth]{img/2_1.png}
% \caption{16x16 vs 32x32 vs 64x64 using 1/16 Dataset}
% \label{fig:capsule_imagedatasize_1_16}
% \end{subfigure}
% %
% %\bigskip
% \begin{subfigure}{\linewidth}
% \includegraphics[width=0.9\textwidth]{img/2_2.png}
% \caption{16x16 vs 32x32 vs 64x64 using 1/8 Dataset}
% \label{fig:capsule_imagedatasize_1_8}
% \end{subfigure}
% %\end{figure}
% %
% %\begin{figure}
% % \ContinuedFloat

% \begin{subfigure}{\linewidth}
% \includegraphics[width=0.95\textwidth]{img/2_3.png}
% \caption{16x16 vs 32x32 vs 64x64 using 1/4 Dataset}
% \label{fig:capsule_imagedatasize_1_4}
% \end{subfigure}
% \end{figure}

% \begin{figure}
% \ContinuedFloat
% \begin{subfigure}{\linewidth}
% \includegraphics[width=0.95\textwidth]{img/2_4.png}
% \caption{16x16 vs 32x32 vs 64x64 using 1/2 Dataset}
% \label{fig:capsule_imagedatasize_1_2}
% \end{subfigure}
% % \end{figure}

% % \begin{figure}
% % \ContinuedFloat


% \begin{subfigure}{\linewidth}
% \includegraphics[width=0.95\textwidth]{img/2_5.png}
% \caption{16x16 vs 32x32 vs 64x64 using All Dataset}
% \label{fig:capsule_imagedatasize_1_1}
% \end{subfigure}
% \caption{Capsule Networks on Different Image Sizes}
% \label{fig:MLP_LSTM_TLModels}
% \end{figure}




==> figure6.tex <==
\begin{figure}[!htb]
  \centering
  \includegraphics[width=0.5\textwidth]{img/7_1}
  \caption{Demonstration of Capsule Networks vs Transfer Learning Models}
  \label{fig:demo}
\end{figure}
